Hybrid Rebeca Revisited

Hybrid Rebeca is a modeling framework for asynchronous event-based cyber-physical systems (CPSs). In this work, we extend Hybrid Rebeca to allow the modeling of non-deterministic time behavior. Besides the syntactical extension, we formalize the semantics of the extended language in terms of Timed Transition Systems, and adapt a reachability analysis algorithm originally designed for hybrid automata to be applicable to Hybrid Rebeca models. We prove the soundness of our approach and illustrate its applicability on a case study. The case study demonstrates that our dedicated algorithm is clearly superior to the alternative approach of transforming Hybrid Rebeca models to hybrid automata as an intermediate model and then applying the original reachability analysis method to this intermediate transformed models.

==> backup.tex <==
\section{Introduction}\label{sec::intro}
Cyber-Physical Systems (CPSs) are usually composed of distributed discrete controllers interacting with physical environment via networked communication. Nowadays, CPSs are ubiquitous in safety-critical situations such as automotive, manufacturing, and transportation. It is important to verify the safety properties of such \textit{Hybrid systems} at design time before their implementation. Formal verification can be useful for this purpose,  %is a suitable technique that verifies the safety properties on a mathematical model specifying the CPS under consideration. By this approach, we compute all reachable states of the model to inspect whether an unsafe state (specified by the safety property) is included.
and \textit{Hybrid automata} is a widely used mathematical model for modeling hybrid systems supported by many automated reachability analysis tools. However, modeling such systems by hybrid automata is not easy. 

%Two important aspects of application of this approach are the model and analysis (computing the reachable states of model). We introduced 
We introduced Hybrid Rebeca in \cite{jahandideh2018hybrid,SoSym}, as an extension of (Timed) Rebeca \cite{sirjani2004modeling,aceto2011modelling}, to faithfully model asynchronously event-based CPSs.   Rebeca provides an operational interpretation of the actor model through a Java-like syntax. %Its timed extension supports modeling of the computation time, and network delay for message communication. Hybrid Rebeca, extends Timed Rebeca with continuous behaviors based on our extended actor model, and the explicit network entity.
Actors, called rebec in this language, are units of concurrency that can only communicate by asynchronous message passing. Each actor is equipped with a mailbox in which the received messages are buffered. The computational model of actors provides a suitable level of abstraction for cyber/physical components and the network to realize the full potential of CPSs. This formalism allows modeling the continuous and discrete aspects of CPSs in a unified way by introducing physical rebecs as an extension of software rebecs with real-valued variables and modes in which the physical dynamics are specified. These modes resemble the location of hybrid automata. %To compute all reachable states over a bounded time horizon and finitely many jumps for a Hybrid Rebeca model with linear dynamics, first a monolithic hybrid automaton is derived from the model. 
To verify the safety properties of a Hybrid Rebeca model, we first derive a monolithic hybrid automaton from the model and then conduct a reachability analysis to inspect the reachability of an unsafe state. As it is well-known the problem of computing the reachable states of a hybrid automaton is undecidable \cite{alur1995algorithmic} as the non-linear differential equations governing the dynamics of real-valued variables cannot be solved. There are many algorithms that approximately solve such equations and compute an over-approximation for the reachable state set in a bounded time interval. If the over-approximated set does not contain any unsafe state, then we can conclude that the system is safe. Most of these algorithms follow a scheme called flowpipe construction \cite{Zha92}. The analysis of a system modeled using Hybrid Rebeca has been demonstrated to be more efficient compared to one modeled with Hybrid Automata \cite{SoSym}. In this approach, the reachability analysis of a Hybrid Rebeca model depends on the derivation of its corresponding hybrid automaton. The number of locations in the derived automata increases exponentially as the number of discrete variables in the software rebecs or the size of the rebec mailbox increases. %, and sometimes it becomes impossible to construct the automata, 
This makes it infeasible to verify complex systems. We remark that the reachability analysis of a hybrid automaton is generally time-bounded and the computation of all locations may not be needed as they may not be reached within the given time-bound. In our new approach, we propose a reachability analysis algorithm on Hybrid Rebeca models directly, with no need to compute hybrid automation as an intermediate model. 



We revise Hybrid Rebeca in both modeling and analysis aspects. For modeling a wide range of CPSs, supporting non-deterministic time behavior is required. For example, the delay of communication or completion of a cyber computation has non-deterministic time behavior. Furthermore, physical rebecs may have non-deterministic behavior due to imprecision in measuring values that affect their behavior (this is modeled through non-deterministic behavior on staying in a mode or leaving it when a guard holds). For instance, we can model the behavior of a smart sensor that non-deterministically decreases the temperature when it exceeds a limit. %send it to a controller and then decrease it. %as we don't know when a sensor measures the temperature, we define a non-deterministic behavior in the mode evolving the temperature or sending the value to the controller. %The sensor non-deterministically follow its dynamic (which changes the temperature) or stops its dynamics by sending the temperature.
We extend Hybrid Rebeca to support modeling non-deterministic time behaviors, realized by the notion of \emph{time intervals}, and allowing non-deterministic behavior for physical rebecs (whether staying or exiting a mode). For the analysis, instead of generating hybrid automata and then computing their reachable states, we compute the reachable states of a Rebeca model directly. %As it is well-known the problem of computing the reachable states of a hybrid automaton is undecidable \cite{alur1995algorithmic} as the non-linear differential equations governing the dynamics of real-valued variables cannot be solved. There are many algorithms that approximately solve such equations and compute an over-approximation for the reachable state set in a bounded time interval. If the over-approximated set does not contain any unsafe state, then we can conclude that the system is safe. Most of these algorithms follow a scheme called flowpipe construction \cite{Zha92}. %%% Given a bounded time horizon $[0,\Delta]$, an over-approximation of the reachable set within $[0,\Delta]$ is iteratively computed as sets of $\mathcal{F}_1,\ldots,\mathcal{F}_N$ %such that $\mathcal{F}_i$ for each $1\le i\le N$ is an 
%%% representing over- approximation of the reachable set over %a time segment in 
%%% $[0,\Delta]$. %, it is also called a flowpipe over-approximation. %There are many suitable representations for flowpipe over-approximations that among then Taylor model is suitable for non-linear dynamics \cite{Taylor}.

%For modeling a wide-range of CPS, presenting non-deterministic behavior over continuous variables is required. For example, the delay of communication or execution of a task have non-deterministic time behavior. A sensor communicate with the controller when temperature is within a bound as we cannot set an exact value for the temperature when the sensor measures.  We extend Hybrid Rebeca to support modeling non-deterministic time behaviors, realized by the notion of Time intervals. The semantics of this extension is defined in terms of extended Interval Time Transition System (eITTS) which is developed based on the standard semantics of Timed-Rebeca. In eITTS, instead of a real value for each continuous variable, real intervals are associated with such variables in each system state. For those values of real variables communicated from physical to software actors leading to an equivalent behavior, we merge those states together by presenting the variables with real intervals. Since the value of real variables depends on time, we represent them by flowpipe.

Given a Hybrid Rebeca model, we seek to over-approximate the set of the states that is reachable in a bounded time horizon $[0,\Delta]$ and with at most $J$ depth of the semantic model, where $\Delta$ and $J$ are user-specified. The bound on the depth is needed when there are many state changes in a small time interval.  We first give the semantic model of the extended Hybrid Rebeca in terms of a Timed Transition System (TTS) with immediate transitions (taken in zero time) and time-progressing transitions. % which is developed based on the standard semantics of Timed-Rebeca.
We then adapt the reachability analysis of hybrid automata \cite{flow} to manage time-progressing transitions. As time advances, the real-valued variables of physical rebecs are approximated using the flowpipe construction algorithm from hybrid automata. The termination of the algorithm is ensured since we bound the time horizon as well as the jump depth.


We define the semantic model of extended Hybrid Rebeca based on the standard semantics of Timed-Rebeca, i.e., TTSs. The global states of a model are defined by the local states of software and physical rebecs and the global time. The local states of rebecs are defined based on their local variable values and message queues. Furthermore, the local states of physical rebecs contain a mode that specifies differential equations, invariant, and a guard. % that govern the dynamics of real-valued variables. 
The invariant of a mode indicates how long a physical rebec remains in a mode while a guard expresses the condition for changing the mode. We can abstract away the concrete values of real values from the local states by considering the mode of physical rebecs. Such abstraction allows us to consider the local states of physical rebecs equal when they only differ in their variable values. We merge those states so that the local states of their rebecs are equal but the global time is different by converting the global time into an interval and associating an interval to the real variables based on the global time interval.  
We represent  all messages that a physical rebec can send within an interval with different real-valued parameters by one message by aggregating their parameter  %flowpipes (which is the solutions of the dynamics of the real variable) 
and arrival times into intervals. We provide a set of operational semantic rules that derive TTSs with appropriate interval values. The proposed rules are designed based on the occurrences of events leading to state changes such as taking a message from a mailbox by a rebec or executing statements for processing messages. %, and resuming computations. %We also aggregate all messages that a physical rebec can send to a reactive rebec within a continuous range of time. So, the arrival time of messages in mailboxes is also an interval. 
%FG A rebec handles a received message from its mailbox if its arrival time interval coincides with the global time interval. A message is either handled for those arrival times within the global time interval, or remained in the mailbox for those arrival times out of the global time interval. %%%This non-deterministic handling of messages is  challenging for messages with real parameters sent by physical rebecs. % carrying the values of real variables. 
%%Since the value of real variables depends on time, instead of an interval value, we should represent such parameters by flowpipe in the messages. 
%FG Upon handling of a message, we execute the message handler while some of parameters may be an interval. So, a conditional statement may have a non-deterministic behavior due to the possibility of its condition expression satisfaction.
Our contributions are summarised as follows:
\begin{itemize}
    \item extending Hybrid Rebeca with time non-deterministic behavior by allowing non-deterministic delay on computation, network communication, or physical mode management;
    \item  providing a semantic model based on the Timed Transition system in which states that only differ by their global time and real-valued variables are merged (while these continuous values are handled by intervals of values); 
    \item Providing the algorithm and tool for state-space generation of Hybrid Rebeca models using existing tools for the reachability analysis of hybrid automata;
    \item illustrating the applicability of our approach through a case study.
\end{itemize}

%intersection of  the real interval of a parameter by using its flowpipe with respect to the length of global time interval.

%The structure of the paper is as follows. In Section \ref{sec::pre}, we explain hybrid automata and its flowpipe construction algorithm. We explain the revised Hybrid Rebeca syntax and semantic model in terms of eITTSs in Section \ref{sec::hyb} and our reachability algorithm in Section \ref{sec::hybImp}. We provide an overview of related work in Section \ref{sec::related}. Finally, Section \ref{sec::con} concludes the paper and highlights our research directions in future.




%The computation model of actors provides a suitable level of abstraction to faithfully model distributed event-based asynchronously communicating systems. Actors are units of computation which can only communicate by asynchronous message passing. Each actor is equipped by a mailbox in which the received messages are buffered. We extend the actor-based language Rebeca, with physical behavior to support hybrid systems.
%To implement the extended actor model, we propose \emph{Hybrid Rebeca}, as an extension of (Timed) Rebeca \cite{sirjani2004modeling,aceto2011modelling}. Rebeca provides an operational interpretation of the actor model through a Java-like syntax. Its timed extension supports modeling of the computation time, and network delay for message communication. Hybrid Rebeca, extends Timed Rebeca with continuous behaviors based on our extended actor model, and the explicit network entity.



%Hybrid Rebeca defines two types of classes, software and physical. Software classes are similar to reactive classes in the Rebeca language where the computational behaviors are defined by message servers. Physical classes in addition to message servers, can also contain different modes, where the continuous behaviors are specified. A physical actor (which is instantiated from a physical class) must always have one active mode. This active mode defines the runtime continuous behavior of the actor. By changing the active mode of a physical actor, it's possible to change the continuous behavior of the actor.  The modes of physical classes are similar to the concept of locations in hybrid automata.

%The semantics of Hybrid Rebeca was given in terms of Hybrid Automata. To this aim, we defined the locations of the derived Hybrid automaton by the discrete values of software rebecs, their queue contents, the modes and queue contents of physical rebeca. The transitions are defined by taking messages from their queues, executing the statements of message handlers, and discrete mode changes, and executing statements as a consequence of discrete jumps of physical rebecs. The number of locations may explode

\section{Motivating Example}
 
The locations of the derived Hybrid automaton are defined by the discrete values of software rebecs, their mailbox contents, the modes and queue contents of physical rebeca.   The transitions are defined by taking messages from their queues, executing the statements of message handlers, and discrete mode changes, and executing statements as a consequence of discrete jumps of physical rebecs. The number of locations may explode

\begin{example}
\begin{figure}[h]
	\centering
	\lstinputlisting[language=HRebeca, multicols=2]{"./code/MotiExample.txt"}
	\caption{A model of a room with a heaterWithSensor, controller, and alarm specified in \HR.}
	\label{code::motiExample}
\end{figure}	
	
\end{example}


%backup of Algorithm 2
{\small
\begin{algorithm}
\caption{ over-approximation reachability analysis}
\KwIn{a \HR model $\mathcal{HR}$, a bounded time horizon $\Delta$, maximum jump depth $\mathcal{J}$, and step size $\TimeStep$% and Taylor series order $\TaylorSeriesOrder$
}
\KwOut{over-approximation of the reachable set of $\mathcal{HR}$'s states% within time interval $\generalIntv{i}{0}{\Delta}{i}$
}
\label{alg::HybridRebecaReachabilityAnalysisAlgorithm}
%--------------------------

$Queue \leftarrow \emptyset$\;
$s_0\leftarrow{\it makeInitialState}(\mathcal{HR})$\; 
$R \leftarrow {\it executeNTPSOS}(s_0)$ \;
\ForEach{$r \in R$} {
	$Queue.equeue(r,\mathcal{J})$
}
\While{$Queue$ is not empty} { 
$\{s:(RS,PS,GT),\mathcal{J}\} \leftarrow Queue.dequeue()$\;
\If{$(\mathcal{J}==0)\vee (GT_{\it up}==\Delta)$}{continue;}


$GT'\leftarrow {\it progressTime}(GT_{\it low},GT_{\it up},{\it EET}_1,{\it EET}_2)$ \tcp*{ where $\ET={\it events}(s)\cup \{GT_{up}+\gamma,\Delta\}$}
\ForEach{$(p,ps)\in PS$}
  { 
  	%\If{${\it flows}.{\it empty}(ps.\mathfrak{m},ps.\sigma)$}
  	${\it ComputeFlowpipes}(ps.\mathfrak{m},ps.\sigma,\gamma,\Delta- GT'_{low})$\;
  }
 $PS'\leftarrow {\it updatePhysicalRebecs}(PS,GT')$\;
\If{${\it inv}(PS')$ is not satisfiable}
  {continue;}
$V\leftarrow\{(RS,PS',GT')\}$\;

\ForEach{$(p,ps)\in PS'$} {
	\If{${\it guard}(ps.\mathfrak{m})$ is satisfiable}
	{\ForEach{$v\in V$}
		{$v' \leftarrow {\it new~GlobalState}(v)$\;
		$v'.PS(p).st \leftarrow {\it trigger}(ps.\mathfrak{m})$\;
		$v'.PS(p).\mathfrak{m} \leftarrow {\it none}$\;
		$V.{\it add}(v')$\;
		 }
	}
}
	\ForEach{$v\in V$}
	{
		$S = {\it executeNTPSOS}(v)$\;
		$R \leftarrow R \cup S$\;
		\ForEach{$s\in S$}
		{
			$Queue.equeue(s,\mathcal{J}-1)$;
		}
	}
 
}
\Return $R$;
\end{algorithm}
}

----

A Rebeca model has two parts : reactive and physical parts. We address the problem of state-space generation for a hybrid model with time continuous model by combining the ideas from both communities. The state space of the reactive part can be generated based on the occurrence of events by considering time intervals that in each interval an event can occur. The state space of the physical part can be constructed by considering small time intervals based on a step size in which the values of approximated. 

The reachability algorithm of hybrid automata combines the ideas by changing a state (based on the guards of the transition) after updating values of for a small time interval. Our reachability algorithm selects the time intervals based on the occurrence of events and a step size and updating the two parts concurrently. The advantage of our approach to the reachability analysis of the corresponding monolithic hybrid automaton is that our approach supports true concurrency. %In the monolithic hybrid automata, once a discrete jump is possible for a physical rebec, the trigger of its modes are immediately executed. Another physical rebec or a resumed reactive rebec 
Changing the mode of a physical rebec, resuming a rebec after a computation delay, and the delivery of a message after a network delay are modeled by discrete jumps in the monolithic hybrid automaton. After the occurrence of each discrete jump, the entering location is an urgent location forcing the physical rebec processes its triggers, the resumed rebec continues its execution until another computation delay is reached or the message processing finishes, the message is immediately handled by the receiving rebec. In other words, the monolithic hybrid automaton results in coarse execution of events and disallows concurrent execution of rebecs.

% difference between two semantics theory and tool
The effect of physical part on the reactive part is considered more precisely. A reactive rebec may behave based on the values it receives from the physical part. By combining the messages that a rebec can send to a reactive rebec 

%conclusin 
We compute the behavior of the conditional statements more precisely based on the intersection of float values and the condition expressions using Hypro.

%tool implementation
We have not used the intersect of Hypro in this implementation. This tool implementation aims at inspection of the feasibility of our approach. Improving the implementation of tool and measuring the precision of its results in comparison with the monolithic hybrid models or the scalability of our approach is among of our future work. 

%conclusion
If a Hybrid Rebeca model has no physical part, the step size can be adjusted to a big value allowing its analysis to be conducted based on the occurrences of events. When ODEs of the physical part has dynamic behavior, the step size can be adjusted to a small value. Dynamic adjustment of the step size is among of our future work.  

%conclusion
In this implementation we considered one step size for managing the reactive and physical parts. We can improve the analysis by considering two step size.
